CodeV: Empowering LLMs with HDL Generation through Multi-Level Summarization

The design flow of processors, particularly in hardware description languages (HDL) like Verilog and Chisel, is complex and costly. While recent advances in large language models (LLMs) have significantly improved coding tasks in software languages such as Python, their application in HDL generation remains limited due to the scarcity of high-quality HDL data. Traditional methods of adapting LLMs for hardware design rely on synthetic HDL datasets, which often suffer from low quality because even advanced LLMs like GPT perform poorly in the HDL domain. Moreover, these methods focus solely on chat tasks and the Verilog language, limiting their application scenarios. In this paper, we observe that: (1) HDL code collected from the real world is of higher quality than code generated by LLMs. (2) LLMs like GPT-3.5 excel in summarizing HDL code rather than generating it. (3) An explicit language tag can help LLMs better adapt to the target language when there is insufficient data. Based on these observations, we propose an efficient LLM fine-tuning pipeline for HDL generation that integrates a multi-level summarization data synthesis process with a novel Chat-FIM-Tag supervised fine-tuning method. The pipeline enhances the generation of HDL code from natural language descriptions and enables the handling of various tasks such as chat and infilling incomplete code. Utilizing this pipeline, we introduce CodeV, a series of HDL generation LLMs. Among them, CodeV-All not only possesses a more diverse range of language abilities, i.e. Verilog and Chisel, and a broader scope of tasks, i.e. Chat and fill-in-middle (FIM), but it also achieves performance on VerilogEval that is comparable to or even surpasses that of CodeV-Verilog fine-tuned on Verilog only, making them the first series of open-source LLMs designed for multi-scenario HDL generation.

==> sections/11_authors.tex <==

\vspace{-40pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author/zhaoyang.jpg}}]{Yang Zhao}
%
received a B.E. degree from Xiamen University, Xiamen, China, in 2024.
He is now a Master's student at the Institute of Computing Technology (ICT), Chinese Academy of Sciences (CAS), in Beijing, China. 
His research interests include machine learning and register-transfer level code generation.
\end{IEEEbiography}
%
 \vspace{-15pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author/huangdi.jpg}}]{Di Huang}
received a B.S. degree from Tsinghua University, Beijing, China, and a Ph.D. degree from the University of Chinese Academy of Sciences, Beijing, China, in 2018 and 2023, respectively. He is currently a postdoctor at State Key Laboratory of Processors, Institute of Computing Technology (ICT), Chinese Academy of Sciences (CAS), Beijing, China. His research interests include deep learning and program synthesis.
\end{IEEEbiography}
%
 \vspace{-15pt}

\begin{IEEEbiography}[{\includegraphics[width=1.1in,height=1.25in,clip,keepaspectratio]{author/lichongxiao.jpg}}]{Chongxiao Li}
%
received his B.E. degree from Shanghai Jiao Tong University, Shanghai, China, in 2020.
He is currently pursuing a PhD degree at the Institute of Computing Technology (ICT), Chinese Academy of Sciences (CAS), Beijing, China.
His research interests include machine learning and computer architecture.
\end{IEEEbiography}
%
 \vspace{-15pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author/jinpengwei.jpg}}]{Pengwei Jin}
%
received the B.S degree from Tsinghua University, Beijing, China in 2020. Currently he is working toward the PhD degree in the Institute of Computing Technology (ICT), Chinese Academy of Sciences, Beijing (CAS), China, and the University of Chinese Academy of Science, Beijing, China. His current research interests include program synthesis and domain-specific hardware architectures.
\end{IEEEbiography}
%
 \vspace{-15pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author/songmuxin.jpg}}]{Muxin Song}
received a B.E. degree from China University of Geosciences, Wuhan, China, in 2023.
He is now a Master's student at the School of Information Science and Technology, ShanghaiTech University, Shanghai, China. 
His research interests include deep learning and register-transfer level code generation.
\end{IEEEbiography}
%
 \vspace{-15pt}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author/xuyinan.png}}]{Yinan Xu}
%
received a B.Eng. degree in computer science and technology from the University of Chinese Academy of Sciences, Beijing, China, in 2019. He is currently a Ph.D. candidate at the State Key Lab of Processors, Institute of Computing Technology, Chinese Academy of Sciences, and the University of Chinese Academy of Sciences, Beijing, China. His research interests include the agile development of processors and open-source computer architecture. Contact him at xuyinan@ict.ac.cn.
\end{IEEEbiography}
%
 \vspace{-15pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author/nanziyuan.jpg}}]{Ziyuan Nan}
%
Ziyuan Nan received a B.S. degree from Beihang University, Beijing, in 2021. He is currently a Ph.D. student at the Institute of Computing Technology (ICT), Chinese Academy of Sciences (CAS), Beijing. His research interests include deep learning and program synthesis.
\end{IEEEbiography}
%
 \vspace{-15pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author/gaomingju.jpg}}]{Mingju Gao}
received a B.E.degree from University of Chinese Academy of Sciences (UCAS), China, in 2023. He is now a Master's student at the Institute of Computing Technology (ICT), Chinese Academy of Sciences (CAS), in Beijing, China. His research interests include deep learning and  program synthesis.
\end{IEEEbiography}
%
 \vspace{-15pt}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author/matianyun.jpg}}]{Tianyun Ma}
%
received the B.S degree from Tsinghua University, Beijing, China in 2020. 
Currently he is working toward the PhD degree in the University of Science and Technology of China, Hefei, China.
His current research interests include machine learning and domain-specific hardware architectures.
\end{IEEEbiography}
%
 \vspace{-15pt}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author/qilei.jpg}}]{Lei Qi}
%
received his B.E. degree from Beijing University of Posts and Telecommunications, Beijing, China in 2023. He is currently pursuing his M.S. degree at University of Science and Technology of China, Hefei, China. His research interests include model compression and code generation.
\end{IEEEbiography}
%
 \vspace{-15pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author/panyansong.png}}]{Yansong Pan}
%
received the bachelor’s degree from the Department of Electronic Engineering, Tsinghua University, China, in 2020. He is currently working toward the Ph.D. degree in computer systems organization at the Institute of Computing Technology, Chinese Academy of Sciences (ICT-CAS). His research interests include reinforcement learning and meta learning.
\end{IEEEbiography}
%
 \vspace{-15pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author/zhangzhenxing.jpg}}]{Zhenxing Zhang}
received his B.S. degree in information and computaional science from the University of Science and Technology of China, Hefei, in 2017, where he is currently pursuing his Ph.D. degree. He is also a visiting student at the State Key Laboratory of Processor, Institute of Computing Technology, Chinese Academy of Sciences, Beijing. His current research interests include computer architecture and parallel computing.
\end{IEEEbiography}
%
 \vspace{-15pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author/zhangrui.jpg}}]{Rui Zhang}
(Member, IEEE) received the Ph.D.
degree in computer application technology from
the Institute of Computing Technology, Chinese
Academy of Sciences, China, in 2019. She is currently an Associate Professor with the Institute of
Computing Technology, Chinese Academy of Sciences, China. Her research areas include computer
vision, large multimodal models, and embodied
artificial intelligence.
\end{IEEEbiography}
%
 \vspace{-15pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author/zhangxishan.jpg}}]{Xishan Zhang}
%
Xishan Zhang received the B.S. degree from the Department of Information Security, Shanghai Jiao Tong University, Shanghai, China, in 2011, and the Ph.D. degree from the Institute of Computing Technology (ICT), Chinese Academy of Sciences (CAS), Beijing, China, in 2017. She is currently an Associate Professor with ICT, CAS. Her current research interests include deep learning and multimedia.
\end{IEEEbiography}
%
 \vspace{-15pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author/duzidong.jpg}}]{Zidong Du}
%
(Member, IEEE) received his B.E. degree from the Department of Electronic Engineering, Tsinghua University, Beijing, China, in 2011, and the Ph.D. degree from ICT, CAS, Beijing, in 2016. He is currently a professor at Intelligent Processor Research Center, ICT, CAS. His research interests mainly focus on novel architecture for artificial intelligence, including deep learning processors, inexact/approximate computing, neural network architecture, neuromorphic architecture. He has published over 20 top-tier computer architecture research papers, including ASPLOS, MICRO, ISCA, TC, TOCS, TCAD. 
%
%
\end{IEEEbiography}
 \vspace{-15pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author/guoqi.jpg}}]{Qi Guo}
%
(Member, IEEE) received the B.E. degree in computer science from Tongji University, Shanghai, China, in 2007, and the Ph.D. degree from ICT, CAS, Beijing, China, in 2012. From 2012 to 2014, he was a Staff Researcher at IBM Research, Beijing. From 2014 to 2015, he was a Postdoctoral Researcher with Carnegie Mellon University, Pittsburgh, PA, USA. He is currently a professor with ICT, CAS. His research interests include computer architecture, programming models, and machine learning.
%
\end{IEEEbiography}

\vspace{-15pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author/huxing.jpg}}]{Xing Hu}
%
(Member, IEEE) received the B.S. degree from Huazhong University of Science and Technology, Wuhan, China, and Ph.D. degree from University of Chinese Academy of Sciences, Beijing, China, in 2009 and 2014, respectively. 
She is currently a professor of State Key Laboratory of Processors, Institute of Computing Technology (ICT), Chinese Academy of Sciences (CAS), Beijing, China.
Her current research interests include domain-specific hardware architectures and deep learning system.
\end{IEEEbiography}
%

\vspace{-15pt}

%
%
%
%


\vfill

==> tables/CodeExamples_1.tex <==
\clearpage
\begin{table*}[t]
\caption{Instruction and response examples from the training set of \modelname{}.}
\label{tab:example1}
\centering
\begin{tabular}{p{5cm}|p{10cm}}
\toprule
\textbf{Instruction} & \textbf{Response}\\
\midrule
\vspace{-5\baselineskip}
Design a 16-to-1 multiplexer (MUX16) using Verilog. The multiplexer should take 16 input signals (I0-I15) and a 4-bit select signal (S3, S2, S1, S0). The output signal O should be the selected input signal based on the select signal. Use a case statement to implement the multiplexer logic.&
\begin{minipage}{35em}
\lstset{style=codestyle}
\begin{lstlisting}[language=Verilog]
module MUX16
(
    input      I0, I1, I2, I3, I4, I5, I6, I7, I8, 
    input      I9, I10, I11, I12, I13, I14, I15,
    input      S0, S1, S2, S3,
    output reg O
);
    always @ (*) begin
        case ({S3, S2, S1, S0})
            4'b0000 : O = I0;
            4'b0001 : O = I1;
            4'b0010 : O = I2;
            4'b0011 : O = I3;
            4'b0100 : O = I4;
            4'b0101 : O = I5;
            4'b0110 : O = I6;
            4'b0111 : O = I7;
            4'b1000 : O = I8;
            4'b1001 : O = I9;
            4'b1010 : O = I10;
            4'b1011 : O = I11;
            4'b1100 : O = I12;
            4'b1101 : O = I13;
            4'b1110 : O = I14;
            4'b1111 : O = I15;
        endcase
    end
endmodule
\end{lstlisting}                
        \end{minipage}\\
        \midrule
        \vspace{-7\baselineskip}
        Implement a Verilog module for a relu (Rectified Linear Unit) function. The module should take a clock signal, a reset signal, and a 32-bit signed input signal sum-in. It should output three signals - done, sum-out, and relu-out. The relu function should set all negative values in the input sum-in to zero and leave positive values unchanged. The done signal should indicate when the relu operation is completed, sum-out should pass through the input sum-in, and relu-out should be the result of the relu function. &
        \begin{minipage}{35em}
\lstset{style=codestyle}
\begin{lstlisting}[language=Verilog]
module relu(
        input clock,
        input reset,
        input signed [31:0] sum_in,
        output reg done,
        output signed [31:0] sum_out,
        output [31:0] relu_out
);
        reg [31:0] relu_out_reg;
        reg [31:0] sum_out_reg;
    always @(posedge clock or posedge reset) begin
                if (reset) begin
                        relu_out_reg <=  32'b0;
                        done <= 1'b0;
                end else begin
                        sum_out_reg <= sum_in;
                        if (sum_in < 0)
                                relu_out_reg <=  32'b0;
                        else begin
                                relu_out_reg <=  sum_in;
                                done <= 1'b1;
                        end
                end
        end
        assign relu_out = relu_out_reg;
        assign sum_out = sum_out_reg;
endmodule
\end{lstlisting}
        \end{minipage}\\
        \bottomrule
    \end{tabular}
\end{table*}
\clearpage

==> tables/FIM_nutshell.tex <==
\begin{table*}[t]
\caption{\parbox{0.9\linewidth}{Comparison of our \xname models against various baseline models. }}
\label{tab:FIM_nutshell}
\centering
\footnotesize
%
%
%
{%
\begin{tabular}{ccccllllll}
\toprule
 \multirow{3}{*}{Model}& \multicolumn{9}{c}{NutShell-FIM (\%)} \\
  & \multicolumn{3}{c}{single-line}&    \multicolumn{3}{c}{multi-line}&\multicolumn{3}{c}{random span} \\ 
   &   pass@1& pass@5& pass@10&    pass@1&pass@5&pass@10&pass@1& pass@5&pass@10\\
  \midrule
  CodeLlama & 51.4 & 65.3 & \multicolumn{1}{c}{70.1 } &    17.4 &22.1 &24.9 &14.0 & 18.3 & 20.0 
\\
  DeepSeek-Coder & 48.0 & 60.0 & \multicolumn{1}{c}{62.3 } &    18.6 &23.0 &24.2 &3.3 & 11.4 & 15.2 
\\
  CodeQwen & 58.4 & 66.9 & \multicolumn{1}{c}{68.6 } &    26.7 &35.7 &39.2 &18.0 & 23.9 & 25.0 
\\
  Qwen2.5-coder& 65.4 & 72.9 &  75.7 &    23.0 &29.9 &32.8 &25.1 & 26.4 &27.1 
\\
 \midrule
 CodeV-CodeLlama & 56.7 & 63.0 & \multicolumn{1}{c}{65.6 } &    32.6 &38.4 &40.0 &12.1 & 15.0 &  

 
16.4 
\\
 CodeV-DeepSeek & 59.0 & 71.6 & \multicolumn{1}{c}{76.0 } &    36.7 &45.8 &50.0 &22.7 & 26.6 & 27.9 
\\
  CodeV-CodeQwen & 68.4 & 75.3 &  76.5 &    30.6 &33.5 &34.2 &17.3 & 21.8 &22.7 
\\
  CodeV-Qwen2.5-Coder& 66.6 & 73.8 & \multicolumn{1}{c}{74.3 } &    21.6 &31.9 &36.2 &20.1 & 24.4 & 27.6 \\
 \bottomrule
\end{tabular}%
}
%
\end{table*}


==> tables/comparison_with_mg.tex <==
\begin{table}[ht]
\centering
\footnotesize
\caption{Comparison of MG-Verilog and CodeV-CodeLlama on VerilogEval}
%
\begin{tabular}{c|ccc|ccc}
\hline
\multirow{2}{*}{Models} & \multicolumn{3}{c|}{Machine(\%)} & \multicolumn{3}{c}{Human(\%)} \\
\cline{2-7}
& pass@1 & pass@5 & pass@10 & pass@1 & pass@5 & pass@10 \\
\hline
MG-VerilogBalancedFine-tune & 59.1 & 69.1 & 72 & 28.1 & 37.9 & 41.5 \\
CodeV-CodeLlama-11k & 60.6 & 74.4 & 79.7 & 30.6 & 43.7 & 49.1 \\
\hline
\end{tabular}%
%
\label{tab:comparison_with_mg}
\end{table}

==> tables/comparsion_with_starcoder2.tex <==
\begin{table*}[t]
\centering
%
%
\begin{tabular}{lccc}
\toprule
Model & HumanEval (+) & MBPP(+) & Data Generation Cost (h) \\
\midrule
Starcoder2-Instruct-CL-7B & 71.3 (66.5)                     & 69.6 (59.8) &  80              \\
InverseCoder-CL-7B (ours)        & \textbf{76.2 (72.0)}                     & \textbf{70.6 (60.1)} & \textbf{4}              \\
\bottomrule
\end{tabular}
\caption{The comparison between our method with Starcoder2-Instruct.}
\label{tab:comparsion_with_starcoder2}
\end{table*}


==> tables/fine-tuning_variance.tex <==
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
\begin{table*}[t]
\caption{Variance analysis of fine-tuning results with different seeds.}
\centering
\footnotesize
\setlength{\tabcolsep}{1mm}
{
\begin{tabular}{cccccccccc}
\toprule
\multirow{2}{*}{Models} & \multirow{2}{*}{Temperature} & \multicolumn{3}{c}{VerilogEval-Machine (\%)} & \multicolumn{3}{c}{VerilogEval-Human (\%)} \\
%
& & pass@1 & pass@5 & pass@10 & pass@1 & pass@5 & pass@10 \\
\midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}CodeV-CL-10K\end{tabular}} 
& 0.2 & \textbf{58.94$\pm$1.06} & 66.08$\pm$1.70 & 68.28$\pm$1.71 & \textbf{30.98$\pm$1.18} & 38.64$\pm$1.60 & 40.76$\pm$1.63 \\
& 0.5 & \underline{57.76$\pm$0.63} & \underline{71.42$\pm$0.83} & \underline{75.36$\pm$0.95} & \underline{27.94$\pm$0.74} & \textbf{41.02$\pm$0.76} & \underline{45.30$\pm$0.76} \\
& 0.8 & 53.74$\pm$1.35 & \textbf{72.98$\pm$1.06} & \textbf{78.08$\pm$0.94} & 23.86$\pm$1.10 & \underline{40.20$\pm$0.81} & \textbf{45.92$\pm$1.21} \\
\bottomrule
\end{tabular}%
}
\label{tab:variance_analysis}
\end{table*}

==> tables/generation_examples_1.tex <==
\begin{table*}[!htb]
    \centering
    \caption{Instruction and response examples of \modelname{}.}
    \begin{tabular}{p{2.5cm}|p{10cm}}
        \toprule
        \textbf{Instruction} & \textbf{Response}\\
        \midrule
        Write a Python script that lists all the files in the current directory. &
        \begin{minipage}{29em}
            Here is a simple Python script that lists all the files in the current directory:

\lstset{style=codestyle}
\begin{lstlisting}[language=Python]
import os

# Get the current directory
current_dir = os.getcwd()

# List all files in the current directory
files = os.listdir(current_dir)

# Print the files
for file in files:
    print(file)
\end{lstlisting}

This script uses the \`{}os\`{} module in Python, which provides a way of using operating system dependent functionality. The \`{}os.getcwd()\`{} function returns the current working directory, and \`{}os.listdir(path)\`{} returns a list containing the names of the entries in the directory given by path.                              
        \end{minipage}\\
        \midrule
        Please show me how to calculate the first ten primes in cpp. &
        \begin{minipage}{29em}
Here is a simple C++ program that calculates the first ten prime numbers:
\lstset{style=codestyle}
\begin{lstlisting}[language=C++]
#include<iostream>
using namespace std;

bool isPrime(int num) {
    if (num <= 1)
        return false;
    for (int i = 2; i * i <= num; i++) {
        if (num %
            return false;
    }
    return true;
}
int main() {
    int count = 0;
    int num = 2;
    while(count < 10) {
        if(isPrime(num)) {
            cout << num << " ";
            count++;
        }
        num++;
    }
    return 0;
}
\end{lstlisting}

This program defines a function \`{}isPrime\`{} that checks if a number is prime. It then uses this function in a loop in the \`{}main\`{} function to find and print the first ten prime numbers.

        \end{minipage}\\
        \bottomrule
    \end{tabular}
    \label{tab:example1}
\end{table*}

==> tables/generation_examples_2.tex <==
\begin{table*}[!htb]
    \centering
    \caption{Instruction and response examples of \modelname{}.}
    \begin{tabular}{p{2.5cm}|p{10cm}}
        \toprule
        \textbf{Instruction} & \textbf{Response}\\
        \midrule
        How to do matrix multiplication in Pytorch? Show me an example. &
        \begin{minipage}{29em}
            Matrix multiplication in PyTorch can be done using the \`{}mm\`{} function from the \`{}torch\`{} module. Here is an example:

\lstset{style=codestyle}
\begin{lstlisting}[language=Python]
import torch

# Create two matrices
matrix1 = torch.tensor([[1, 2, 3], [4, 5, 6]])
matrix2 = torch.tensor([[7, 8], [9, 10], [11, 12]])

# Perform matrix multiplication
result = torch.mm(matrix1, matrix2)

print(result)
\end{lstlisting}

In this example, \`{}matrix1\`{} is a 2x3 matrix and \`{}matrix2\`{} is a 3x2 matrix. The \`{}mm\`{} function performs matrix multiplication on these two matrices and returns a new matrix.

The output will be:

\lstset{style=codestyle}
\begin{lstlisting}[language=Python]
tensor([[ 58,  64],
        [139, 154]])
\end{lstlisting}


        \end{minipage}\\
        \midrule
        Please check if the network can connect to www.example.com using Python. &
        \begin{minipage}{29em}

Sure, you can use the \`{}requests\`{} library in Python to check if a network can connect to \`{}www.example.com\`{}. Here is a simple script:
\lstset{style=codestyle}
\begin{lstlisting}[language=Python]
import requests

try:
    response = requests.get("http://www.example.com")
    response.raise_for_status()
    print("Connection successful")
except requests.exceptions.HTTPError as errh:
    print ("Http Error:",errh)
except requests.exceptions.ConnectionError as errc:
    print ("Error Connecting:",errc)
except requests.exceptions.Timeout as errt:
    print ("Timeout Error:",errt)
except requests.exceptions.RequestException as err:
    print ("Something went wrong",err)
\end{lstlisting}
This script sends a GET request to \`{}www.example.com\`{} and checks for any exceptions that might occur during the request. If the request is successful, it prints ``Connection successful''. If there is an HTTP error, a connection error, a timeout error, or any other type of request exception, it prints the error.

        \end{minipage}\\
        \bottomrule
    \end{tabular}
    \label{tab:example2}
\end{table*}

==> tables/model_comparison.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{lccccc}
    \toprule
    Model                             & Annotation Sources & HumanEval+  & MBPP+ & MultiPL-E \footnotemark & DS-1000 \\
    \midrule
    \multicolumn{4}{l}{\it (unknown annotation sources)} \\
    GPT-3.5-Turbo (Nov 2023)          & Unknown           & 70.7   & 69.7 & 64.9 & - \\
    DeepSeekCoder-33B-Instruct        & Unknown           & 75.0   & 70.1 & 69.2 & - \\
    CodeQwen1.5-7B-Chat               & Unknown           & 78.7   & 69.0 & 72.0  & - \\
    GPT-4-Turbo (April 2024)          & Unknown           & \textbf{86.6} & \textbf{73.3} & \textbf{76.5} & - \\
    \midrule
    \multicolumn{4}{l}{\it (known annotation sources)} \\
    WizardCoder-CL-15B              & GPT-3.5          & 50.6  & 54.2 & - & 29.2 \\
    Magicoder-S-CL-7B               & GPT-4 + GPT-3.5  & 67.7  & 60.1 & 46.1 & 37.5 \\
    Magicoder-S-DS-6.7B             & GPT-4 + GPT-3.5  & 71.3  & \textbf{69.0} & - & -  \\
    OpenCodeInterpreter-DS-6.7B     & GPT-4 + GPT-3.5  & 72.0  & 66.4 & - & -   \\
    \modelname-DS-6.7B \textbf{(ours)} & \textbf{GPT-4 + self-generated} & \textbf{76.8} & \textbf{69.0} & \textbf{62.6} & \textbf{44.2} \\
    \bottomrule
    \end{tabular}
    \caption{Comparisons between \modelname and other well-known Code LLMs in annotation data sources and performances on a diverse range of benchmarks. \modelname surpasses all of the other Code LLMs using the same GPT-4 annotation dataset.}
    \label{tab:annotation_cost}
\end{table*}



==> tables/multi-pl-e.tex <==
\begin{table*}[t]
\centering
%
%
\begin{tabular}{lccccccc}
\toprule
Model                   & Java & JS & C++  & PHP  & Swift & Rust & Avg. \\

\midrule
\multicolumn{8}{l}{\it (Based on \codellamapy-13B)} \\
WizardCoder-GPT4-CL-13B*    & \textbf{55.4} & 64.2 & 55.9 & 52.0 & 49.9 & 53.4 & 55.1 \\
InverseCoder-CL-13B (ours)* & 54.5 & \textbf{65.4} & \textbf{58.1} & \textbf{55.3} & \textbf{52.5} & \textbf{55.6} & \textbf{56.9} \\

\midrule
\multicolumn{8}{l}{\it (Based on \codellamapy-7B)} \\
CodeLlama-7B               & 29.3 & 31.7       & 27.0 & 25.1 & 25.6  & 25.5 & 27.4 \\
CodeLlama-Python-7B        & 29.1 & 35.7       & 30.2 & 29.0 & 27.1  & 27.0 & 29.7 \\
%
Magicoder-S-CL-7B          & 42.9 & 57.5       & 44.4 & 47.6 & 44.1  & 40.3 & 46.1 \\
Magicoder-S-CL-7B*         & 49.8 & \textbf{62.6} & 50.2 & 53.3 & 44.9 & 43.8 & 50.8 \\
WizardCoder-GPT4-CL-7B*    & \textbf{50.4} & 60.7 & 50.6 & 51.6 & 45.6 & \textbf{48.2} & 51.2 \\
InverseCoder-CL-7B (ours)* & 48.7 & 61.9 & \textbf{52.6} & \textbf{55.2} & \textbf{53.0} & 46.1 & \textbf{52.9} \\

\midrule
\multicolumn{8}{l}{\it (Based on DeepSeek-Coder-6.7B)} \\
Magicoder-S-DS-6.7B* & 59.6 & 69.8 & 70.0 & \textbf{64.4} & \textbf{54.4} & 53.6 & 62.0 \\
WizardCoder-GPT4-DS-6.7B*    & \textbf{61.4} & 66.4 & 68.7 & 61.8 & 52.6 & 56.1 & 61.2 \\
InverseCoder-DS-6.7B (ours)*  & 60.7 & \textbf{70.1} & \textbf{70.5} & 63.6 & 53.0 & \textbf{57.4} & \textbf{62.6} \\

\bottomrule
\end{tabular}
\caption{\Passat{1} (\%) results of different \llm{s} on \multiple~\cite{multiple}. The models marked with (*) are evaluated with the same prompt format as training and the following hyperparameter: $\temperature=0.2$, $\topp=0.95$, $\maxLen=4096$, $\nsamples=50$ and $\batchsize=2$ . We report other results consistently from Magicoder paper.}
\label{tab:multilang}
\end{table*}


==> tables/observation_check_exp.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{ccccc}
    \toprule
    Task                  & Prediction   & Label               & WizardCoder-GPT4-CL-7B & WizardCoder-GPT4-DS-6.7B \\
    \midrule
    NL $\rightarrow$ Code & $y'$         & $\hat{y}_{gpt}$    & 73.8 (65.2)         & 82.2 (73.8)         \\
    Code $\rightarrow$ NL & $y$          & $\hat{y}'_{gpt}$   & \textbf{85.2 (73.9)}         & \textbf{87.0 (76.0)}         \\
    \midrule
    NL $\rightarrow$ Code & $y'$         & $y$                 & 69.3 (59.3)         & 77.8 (67.5)         \\
    Code $\rightarrow$ NL & $y$          & $\hat{y}'_{human}$ & \textbf{86.7 (86.7)}         & \textbf{80.0 (80.0)} \\
    \bottomrule
    \end{tabular}
     \caption{\Passat{1} (\%) results on MBPP(+) in observation checking experiments.}
    \label{tab:observation_check_exp}
\end{table*}



==> tables/qlora.tex <==
\begin{table}[t]
\caption{Performance comparison of QLoRA and full parameter fine-tuning on VerilogEval, where "p@k" denotes "pass@k". It shows that the performance of different training methods is similar.}
\centering
\setlength{\tabcolsep}{1mm}
\footnotesize
\begin{tabular}{cccccccc}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Temp.} & \multicolumn{3}{c}{Machine (\%)} & \multicolumn{3}{c}{Human (\%)} \\
%
 &  & p@1 & p@5 & p@10 & p@1 & p@5 & p@10 \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}CodeV-CL\\10K-QLoRA\end{tabular}} & 0.2 & 56.8 & 61.6 & 63.0 & \textbf{33.6} & 39.5 & 41.3 \\
 & 0.5 & 57.3 & 67.0 & 70.0 & \underline{32.9} & \underline{43.8} & \underline{47.4} \\
 & 0.8 & 56.7 & 68.0 & 71.4 & 32.3 & \textbf{43.9} & 46.9 \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}CodeV-CL\\10K-Full\end{tabular}} & 0.2 & \textbf{58.7} & 64.2 & 65.8 & 30.9 & 38.2 & 40.3 \\
 & 0.5 & \underline{58.1} & \underline{71.0} & \underline{74.7} & 27.4 & 40.5 & 45.0 \\
 & 0.8 & 54.4 & \textbf{73.7} & \textbf{78.5} & 24.3 & 41.2 & \textbf{47.8} \\ \bottomrule
\end{tabular}%
\label{tab:performance_qlora}
%
\end{table}

==> tables/sat.tex <==
\begin{table}[ht]
\centering
\footnotesize
\caption{SAT time reduction task compared with BetterV. We report the optimized design’s SAT time proportion to the reference design.}
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{lcccc}
\hline
& b03 & b06 & Spinner & traffic\_light\_example \\
\hline
Ref in BetterV(s) & 1.233 & 0.099 & 1.577 & 0.583 \\
BetterV-base prop. & 101.54\% & 83.84\% & 85.16\% & 85.25\% \\
BetterV-dis prop. & 69.51\% & 78.79\% & 67.47\% & 82.33\% \\
Ref reproduction(s) & 0.979 & 0.137 & 1.327 & 0.516 \\
CodeV-CL prop. & 105.21\% & 101.46\% & 104.75\% & 98.26\% \\
RTLCoder-DS prop. & 102.45\% & 94.16\% & 85.15\% & 93.60\% \\
\hline
\end{tabular}%
}
\label{tab:sat}
\end{table}[]

==> tables/self-consistency.tex <==
\begin{table*}[t]
\small
\centering
\begin{tabular}{lcc}
\toprule
Model                  & Self-Consistency Pass@1 on MBPP(+) & \# of removed problems \\
\midrule
CodeLlama-Python       & 42.7 (41.4)                     & 64                    \\
DeepSeek-Coder         & 57.4 (50.6)                     & 68                    \\
\midrule
WizardCoder-GPT4-CL    & 69.0 (65.6)                     & 52                    \\
InverseCoder-CL (ours) & \textbf{76.0 (73.5)}            & 53                    \\
\midrule
WizardCoder-GPT4-DS    & 76.1 (69.7)                     & 48                    \\
InverseCoder-DS (ours) & \textbf{80.4 (75.3)}            & 46                    \\
\bottomrule
\end{tabular}
 \caption{\Passat{1} (\%) results on MBPP(+) in the self-consistency experiment. The generation and evaluation process are the same as the MBPP(+) experiments in Section \ref{sec:main_results} except the canonical solutions. We also report the problems removed due to errors in original answers.}
\label{tab:self-consistency}
\end{table*}

==> tables/self-improve.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{lcc}
\toprule
Model                       & HumanEval (+) & MBPP (+)     \\
\midrule
CodeLlama-Python-7B         & 39.6 (35.4)  & 51.9 (43.7) \\
+$1$ epoch self-generated & 54.3 (49.3)  & 52.9 (44.7) \\
+$2$ epoch self-generated & \textbf{54.9 (50.6)}  & \textbf{54.2 (46.6)} \\
\bottomrule
\end{tabular}
 \caption{\Passat{1} (\%) results on HumanEval~(+) and MBPP~(+) in self-improving  experiments for base model \codellamapy-7B. We report performances of the model finetuned with generated data for $1$ and $2$ epochs. The other hyperparameters are the same as Section \ref{sec:main_results}.}
 \label{tab:self-improve}
\end{table*}

==> tables/table_bottom.tex <==
\begin{table*}[ht]
\centering
\footnotesize
\caption{AIG node reduction task compared with BetterV. We report the optimized design's node count proportion compared to the reference design. Our CodeV fails to optimize alone but shows significant node reduction after combining with EDA optimizations.}
\label{tab:comparison}
\resizebox{1\textwidth}{!}{%
\begin{tabular}{cccccccc}
\toprule
\textbf{Problem} & \textbf{Ref} & \textbf{BetterV-base prop.(\%)} & \textbf{BetterV-dis prop.(\%)} & \textbf{RTLCoder-ds prop.(\%)} & \textbf{RTLCoder-ds+opt prop.(\%)} & \textbf{CodeV-cl prop.(\%)} & \textbf{CodeV-cl+opt prop.(\%)} \\
\midrule
ece241\_203\_q8 & 657 & 50.76 & 38.86 & 101.52 & 2.59 & 100.00 & 2.59 \\
m2014\_q6 & 1370 & 50.56 & 50.04 & 100.00 & 2.34 & 88.39 & 2.34 \\
review2015\_count1k & 487 & 101.31 & 82.67 & 105.85 & 16.53 & 103.88 & 15.79 \\
timer & 498 & 59.10 & 49.66 & 102.45 & 39.56 & 100.00 & 39.16 \\
edgedetect2 & 58 & 327.41 & 81.72 & 124.48 & 100.00 & 100.00 & 100.00 \\
count1to10 & 325 & 81.94 & 73.94 & 104.83 & 10.92 & 108.62 & 10.15 \\
2013\_q2afsm & 826 & 37.38 & 35.91 & 100.07 & 3.64 & 100.00 & 3.63 \\
dff8p & 50 & 84.60 & 75.60 & 100.00 & 38.00 & 100.00 & 38.00 \\
fsm3comb & 844 & 19.89 & 12.37 & 100.00 & 1.42 & 100.00 & 1.42 \\
rule90 & 6651 & 186.97 & 68.21 & 100.00 & 92.26 & 100.04 & 92.26 \\
mux256to1v & 2376 & 102.68 & 23.45 & 84.99 & 0.14 & 71.44 & 2.61 \\
fsm2 & 389 & 47.95 & 31.34 & 100.00 & 1.03 & 100.00 & 1.03 \\
fsm2s & 396 & 41.34 & 36.39 & 37.37 & 1.52 & 100.23 & 1.52 \\
ece241\_2013 q4 & 2222 & 80.54 & 40.39 & 100.00 & 1.40 & 92.17 & 1.40 \\
count\_clock & 3187 & 78.37 & 69.73 & 100.00 & 16.25 & 100.00 & 16.25 \\
countbcd & 1589 & 58.65 & 53.45 & 100.00 & 12.52 & 100.00 & 12.52 \\
\bottomrule
\end{tabular}%
}
\label{tab:table_bottom}
\end{table*}

==> tables/table_rtop.tex <==
\begin{table}[t]
\caption{Modified lines of code (Mod. LoC), the resulting correct module’s lines of code (Res. LoC), and modified proportions for different modules (Mod. Prop.) shown in Figure~\ref{fig:practical_design}.}
\centering
\setlength{\tabcolsep}{1mm}
\footnotesize
%
\small
\begin{tabular}{ccccc}
\toprule
Design & Module & Mod. LoC & Res. LoC & Mod. Prop.\\
\hline
\multirow{7}{*}{PCES} & sbox & 0.00 & 21.00 & 0.00\% \\
& substitution & 2.67 & 45.00 & 5.23\% \\
& permutation & 0.00 & 65.00 & 0.00\% \\
& sub\_per & 0.00 & 4.00 & 0.00\% \\
& key\_update & 4.67 & 10.33 & 45.45\% \\
& present\_encryptor\_top & 14.67 & 99.67 & 16.76\% \\
\midrule
%
\multirow{8}{*}{ITW} & i2s\_to\_wb\_tx\_if & 38.00 & 42.33 & 89.84\% \\
& sync\_fifo & 38.67 & 75.33 & 51.89\% \\
& i2s\_to\_wb\_tx & 12.00 & 31.33 & 44.53\% \\
& tone\_440\_rom & 0.00 & 7.00 & 0.00\% \\
& i2s\_to\_wb\_dma\_fsm & 9.00 & 55.00 & 16.88\% \\
& i2s\_to\_wb\_fifo\_fsm & 9.67 & 68.33 & 14.50\% \\
& i2s\_to\_wb\_top & 42.67 & 49.33 & 86.46\% \\
& i2s\_to\_wb\_tx\_dma & 30.00 & 30.00 & 100.00\% \\
\bottomrule
\end{tabular}%
%
\vspace{-6pt}
\label{tab:table_rtop}
\end{table}

==> tables/text2code.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{0.5mm}
\centering
\begin{tabular}{lccc}
\toprule
Model                    & HumanEval~(+) & MBPP~(+)     \\
\midrule
\multicolumn{3}{l}{\it (Closed-source Models)}                   \\
GPT-4-Turbo (April 2024) & \textbf{90.2 (86.6)}  & \textbf{85.7 (73.3)} \\
GPT-3.5-Turbo (Nov 2023) & 76.8 (70.7)  & 82.5 (69.7) \\

\midrule 
\multicolumn{3}{l}{\it (Based on \codellamapy-13B)}                   \\
\codellamapy-13B          & 42.7 (38.4)  & 63.5 (52.6) \\
WizardCoder-GPT4-CL-13B      & 76.8 (70.7)  & 73.5 (62.2) \\
InverseCoder-CL-13B (ours)   & \textbf{79.9 (74.4)}  & \textbf{74.6 (63.0)} \\

\midrule 
\multicolumn{3}{l}{\it (Based on \codellamapy-7B)}                   \\
\codellamapy-7B          & 37.8 (35.4)  & 59.5 (46.8) \\
WizardCoder-CL-7B           & 50.6 (45.1)  & 58.5 (49.5) \\
%
Magicoder-S-CL-7B           & 70.7 (67.7)  & \textbf{70.6 (60.1)} \\
WizardCoder-GPT4-CL-7B      & 72.6 (68.9)  & 69.3 (59.3) \\
InverseCoder-CL-7B (ours)   & \textbf{76.2 (72.0)}  & \textbf{70.6 (60.1)} \\


\midrule
\multicolumn{3}{l}{\it (Based on DeepSeek-Coder-6.7B)}                   \\
DeepSeek-Coder-6.7B      & 47.6 (39.6)  & 72.0 (58.7) \\
DeepSeek-Coder-Instruct-6.7B  & 74.4 (71.3)  & 74.9 (65.6) \\
%
Magicoder-S-DS-6.7B           & 76.8 (71.3)  & \textbf{79.4} (\textbf{69.0}) \\
WaveCoder-Ultra-DS-6.7B       & 75.0 (69.5)  & 74.9 (63.5) \\
OpenCodeInterpreter-DS-6.7B   & 77.4 (72.0)  & 76.5 (66.4) \\
%
WizardCoder-GPT4-DS-6.7B      & 77.4 (73.2)  & 77.8 (67.5) \\
InverseCoder-DS-6.7B (ours)   & \textbf{79.9 (76.8)}  & 78.6 (\textbf{69.0}) \\


\bottomrule
\end{tabular}
 \caption{\Passat{1} (\%) results of different \llm{s} on \humaneval{}~(+) and \mbpp{}~(+) computed with greedy decoding. The abbreviations ``CL'' and ``DS'' refer to the base models \codellamapy~and \dscoder, respectively. We set $\batchsize=4$ to evaluate the models trained by ourselves.
 We report other results consistently from the \evalplus~\cite{EvalPlus} Leaderboard in August 2024 and Magicoder \cite{magicoder} paper. 
 }
\label{tab:python-text2code}

\end{table}

==> tables/token_counter.tex <==
\begin{table}[ht]
\centering
\footnotesize
\caption{Number of Tokens Used and Performance Comparison}
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{l|ccc}
\hline
Dataset & No. of tokens in dataset & No. of tokens trained & VerilogEval-Machine (pass@1) \\
\hline
RTLCoder & 19.16M & 57.49M & 61.2 \\
CodeV-27k (ours) & 20.73M & 62.18M & 72.3 \\
CodeV (ours) & 110.30M & 330.91M & 77.6 \\
\hline
\end{tabular}%
}
\label{tab:token_usage_performance}
\end{table}

==> tables/token_distribution.tex <==
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
\begin{table}[t]
\caption{Statistics on token counts for code and descriptions in the dataset, and the proportion of single-module and multi-module code.}
\centering
\footnotesize
\setlength{\tabcolsep}{1mm}
{
\begin{tabular}{ccccc}

\toprule
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Code \\ Tokens \end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}High-level \\ Summaries \\ Tokens\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Detailed \\ Descriptions \\Tokens\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Single-module \\ Code \\ Percentage\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Multi-module \\ Code\\ Percentage\end{tabular}} \\
%
& & & &  \\
& & & &  \\
\midrule
3.94e7 & 2.25e7 & 2.50e7 & 93.1\% & 6.9\% \\
\bottomrule
\end{tabular}%
}

\label{tab:token_distribution}
\end{table}
